PANGAEA: A Global and Inclusive Benchmark for Geospatial Foundation Models

Geospatial Foundation Models (GFMs) have emerged as powerful tools for extracting representations from Earth observation data, but their evaluation remains inconsistent and narrow. Existing works often evaluate on suboptimal downstream datasets and tasks, that are often too easy or too narrow, limiting the usefulness of the evaluations to assess the real-world applicability of GFMs. Additionally, there is a distinct lack of diversity in current evaluation protocols, which fail to account for the multiplicity of image resolutions, sensor types, and temporalities, which further complicates the assessment of GFM performance. In particular, most existing benchmarks are geographically biased towards North America and Europe, questioning the global applicability of GFMs. To overcome these challenges, we introduce PANGAEA, a standardized evaluation protocol that covers a diverse set of datasets, tasks, resolutions, sensor modalities, and temporalities. It establishes a robust and widely applicable benchmark for GFMs. We evaluate the most popular GFMs openly available on this benchmark and analyze their performance across several domains. In particular, we compare these models to supervised baselines (e.g. UNet and vanilla ViT), and assess their effectiveness when faced with limited labeled data. Our findings highlight the limitations of GFMs, under different scenarios, showing that they do not consistently outperform supervised models. PANGAEA is designed to be highly extensible, allowing for the seamless inclusion of new datasets, models, and tasks in future research. By releasing the evaluation code and benchmark, we aim to enable other researchers to replicate our experiments and build upon our work, fostering a more principled evaluation protocol for large pre-trained geospatial models. The code is available at https://github.com/VMarsocci/pangaea-bench.

==> figs_tex/fbps_sample.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{figs/image_fpbs.png} % Replace with your image file
        \caption{Image} 
        \label{fig:fbssubfig1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/label_fpbs.png} % Replace with your image file
        \caption{Ground truth}
        \label{fig:fbpsubfig2}
    \end{subfigure}
    \caption{Example data of \textbf{Five Billion Pixels} (Location: China. Domain: Urban Land Cover).}
    \label{fig:fbps_example}
\end{figure*}

==> figs_tex/sn7_sample.tex <==
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs/sn7_change_sample.png}
%     \caption{SpaceNet 7 sample data: (a) Pre-change Planet image, and (b) Post-change Planet image (c) Built-up area change label.}
%     \label{fig:sn7_sample}
% \end{figure}


\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/sn7_sample_image_t1.png} 
        \caption{Pre-change image}
        \label{subfig:prechange_image}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/sn7_sample_image_t2.png} 
        \caption{Post-change image}
        \label{subfig:postcange_image}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/sn7_sample_change.png} 
        \caption{Building change label}
        \label{subfig:change_label}
    \end{subfigure}
    
    \caption{Example data for the SpaceNet 7 dataset. The pre-change and post-change images represent the first and last cloud-free satellite images in the time series, respectively. The change label visualizes unchanged (black) and changed (white) pixels regarding built-up areas between the two images.}
    \label{fig:sn7-examples}
\end{figure*}

==> figs_tex/wp_pangaea.tex <==
\begin{figure*}[htbp]
    \vspace{-3pt}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/pangaea_fig.png}
    \caption{PANGAEA aims for robust evaluation across diverse downstream datasets and applications.}
    \vspace{-8pt}
    \label{fig:pangaea}
\end{figure*}

==> figs_tex/wp_teaser.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/main_results.jpg}
    \caption{\textbf{Normalized performance comparison of different models across various datasets and training conditions.} The y-axis represents the {normalized performance} across the 11 PANGAEA's datasets, where the best-performing model for each dataset is assigned a value of 1 and the worst-performing model is assigned a value of 0. 
    (a) \textbf{Full Labels}: Models trained on downstream tasks with access to the full labeled dataset. We observe that supervised baselines -- especially UNet -- outperform most of the models; 
    (b) \textbf{Limited Labels (10\%)}: Models trained on downstream tasks with only 10\% of labeled data. In this scenario, some GFMs -- \eg CROMA -- excel and outperform both other GFMs and supervised baselines, although still competitive; 
    (c) \textbf{Multi-Spectral Data}: Results for datasets made exclusively of multi-spectral images, \ie HLS Burn Scars, MADOS, PASTIS-R, Sen1Floods11, Crop Type Mapping-SS, and BioMassters. Multi-spectral datasets tend to use low-resolution images, on which UNet excels. GFMs trained on high-resolution images, \eg Scale-MAE, underperform in this setting that requires both spatial and spectral information;
    (d) \textbf{High-Resolution Data}: Results for high-resolution datasets, \ie xView2, FiveBillionPixels, DynamicEarthNet, and SpaceNet 7. They are made of either RGB or RGB-NIR imagery. In this setting, most GFMs pre-trained on lower-resolution imagery fall behind, except CROMA and DOFA. On the other hand, GFMs pre-trained on high-resolution images and UNet perform well.}
    \label{fig:teaser}
\end{figure*}

==> figs_tex/xview2_sample.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/moore-tornado_00000110_pre_disaster_1_0.png} 
        \caption{Pre-disaster image}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/moore-tornado_00000110_post_disaster_1_0.png} 
        \caption{Post-disaster image}
        \label{fig:sub2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/moore-tornado_00000110_post_disaster_1_0_label_noalpha.png} 
        \caption{Building damage label}
        \label{fig:sub3}
    \end{subfigure}
    
    \caption{Example data of \textbf{xView2} (Location: Global. Domain: HADR.). The image is taken from the 2013 Moore Tornado. Different colors in the label indicate different building damage classes.}
    \label{fig:xview2-examples}
\end{figure*}

==> tabs/extensive_ai4smallfarms_finetune.tex <==
\begin{table*}[htbp]
\centering
\caption{Performance comparison of finetuned CROMA and SSL4EO\_MAE models on the AI4SmallFarms dataset.}
\label{tab:finetune_results}
\begin{tabularx}{\textwidth}{llYYYY}
\toprule
Model & Class & IoU$\uparrow$ & F1$\uparrow$ & prec$\uparrow$ & rec$\uparrow$ \\
\midrule
\multirow{3}{*}{CROMA Finetuned} & Background & 23.799 & 38.448 & 24.969 & 83.549 \\
& Crop Field & 25.755 & 40.961 & 84.941 & 26.987 \\
& Mean & 24.777 & 39.705 & 54.955 & 55.268 \\
\midrule
\multirow{3}{*}{SSL4EO\_MAE Finetuned} & Background & 21.895 & 35.924 & 22.899 & 83.307 \\
& Crop Field & 25.568 & 40.724 & 85.946 & 26.684 \\
& Mean & 23.731 & 38.324 & 54.423 & 54.995 \\
\bottomrule
\end{tabularx}
\end{table*}

==> tabs/extensive_biomass2.tex <==
\begin{table*}[htbp]
\caption{Biomassters results. Comparison of best and worst performing foundation models with UNet and ViT baselines, all in a fully supervised setting. The UNet baseline model has no temporal strategy.}
\centering
\begin{tabularx}{\textwidth}{lcYYYYYYYYY}
\toprule
         & & \multicolumn{3}{c}{Uni-temporal} & \multicolumn{6}{c}{Multi-temporal} \\ 
                   & & & & & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{L-TAE} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule{9-11}
         Model & Modality & 10\% & 50\% & 100\% & 10\% & 50\% & 100\% & 10\% & 50\% & 100\% \\
\midrule         
         
         RemoteCLIP     & optical & 54.84	& 52.39	& 51.58 & 53.21	& 49.17	& 48.66	& 50.00	& 47.22	& 46.34 \\
         CROMA  & optical & 47.83 & 46.07 & 45.11 & OOM & OOM & OOM & OOM & OOM &OOM \\
         \midrule
         % ---------------------------------- BASELINES -------------------------------- \\ 
         UNet Baseline & optical  & 44.83 & 41.24 & 40.83&   40.39 & 36.72 & 35.67&   40.39 & 36.72 & 35.67\\  % NO MT strategy           
         ViT Baseline  & optical  & 49.13 & 46.22 & 43.77&	46.19 & 39.96 & 40.94&    44.89& 39.56 & 38.55 \\ 

\bottomrule
\end{tabularx}
\label{tab:extensive-biomass2}
\end{table*}




==> tabs/extensive_hlsburnscars_best_worst.tex <==
% \begin{table}[H]
% \centering
% \caption{Results for the ablation study on HLS Burn Scars, comparing RemoteCLIP (worst) and Prithvi (best) with end-to-end fine-tuning of encoder and decoder.}
% \label{tab:ablation_hlsburnscars}
% \renewcommand{\arraystretch}{1.5} 
% \begin{adjustbox}{width=1\textwidth}
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{l|ccccc|ccccc}
% \toprule
%  & \multicolumn{5}{c|}{RemoteCLIP} & \multicolumn{5}{c}{Prithvi} \\
% Metric & mIoU & m-F1 & m-Precision & m-Recall & m-Accuracy & mIoU & m-F1 & m-Precision & m-Recall & m-Accuracy \\
% \midrule
% Not burned     & 91.859 & 95.757 & 96.340 & 95.181 & 92.253 & 96.918 & 98.435 & 98.146 & 98.726 & 97.168 \\ 
% Burn scar      & 38.404 & 55.496 & 52.183 & 59.257 & 65.132 & 74.114 & 85.133 & 87.585 & 82.814 & 85.516 \\ 
% Mean  & 65.132 & 75.626 & 74.262 & 77.219 & 92.253 & 85.516 & 91.784 & 92.865 & 90.770 & 97.168 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}

\begin{table*}[htbp]
\centering
\caption{Results for the ablation study on HLS Burn Scars, comparing RemoteCLIP (worst) and Prithvi (best) with end-to-end fine-tuning of encoder and decoder.}
\label{tab:ablation_hlsburnscars}
\begin{tabularx}{\textwidth}{lYYYYYYYYYY}
\toprule
 & \multicolumn{5}{c}{RemoteCLIP} & \multicolumn{5}{c}{Prithvi} \\
 \cmidrule(lr){2-6} \cmidrule(lr){7-11}
& mIoU & m-F1 & m-pre & m-rec & m-acc & mIoU & m-F1 & m-prec & m-rec & m-acc \\
\midrule
Not burned     & 91.86 & 95.76 & 96.34 & 95.18 & 92.25 & 96.92 & 98.44 & 98.15 & 98.73 & 97.17 \\ 
Burn scar      & 38.40 & 55.50 & 52.18 & 59.26 & 65.13 & 74.11 & 85.13 & 87.59 & 82.81 & 85.52 \\ 
Mean  & 65.13 & 75.63 & 74.26 & 77.22 & 92.25 & 85.52 & 91.78 & 92.865 & 90.770 & 97.17 \\
\bottomrule
\end{tabularx}
\end{table*}


==> tabs/extensive_sen1floods11.tex <==
\begin{table*}[htbp]
\centering
\caption{Sen1Floods11 results with 100\% of the data, best results in \textbf{bold}, second best \underline{underlined}. The results in the last four columns are for the foreground class (water).}
\label{tab:extensive-floods}
\resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccccccccc}
    \toprule
        Model &  Modality & mIoU$\uparrow$ & m-F1$\uparrow$ & m-prec$\uparrow$ & m-rec$\uparrow$ & m-acc$\uparrow$& IoU $\uparrow$ & F1$\uparrow$ &  prec$\uparrow$ & rec$\uparrow$ \\
        \midrule
        CROMA  &optical    & \underline{90.89}&	\underline{95.09}&	 \textbf{94.33} &	\underline{95.90}&	\underline{97.89}&	\underline{84.15}&	\underline{91.39}&	 \textbf{89.58}&	\underline{93.28} \\
        DOFA  &optical & 88.78&	93.86&	92.91&	94.86&	97.35&	80.54&	89.22&	86.98&	91.57 \\
        GFM-Swin &optical & 72.60	&82.51	&78.34	&88.99	&93.36	&52.36	&68.73	&58.30	&83.70\\
        Prithvi &optical   & 90.37	&94.80	&94.01	&95.62	&97.76	&83.26	&90.86 &89.00	&92.81 \\
        RemoteCLIP  &optical&74.26&	83.83&	79.44&	90.70&	93.84&	55.18&	71.11&	60.19&	86.89 \\
        SatlasNet &optical & 90.30&	87.51&	92.5&	95.71&	97.75&	83.12&	90.79&	86.00&	92.53\\
        Scale-MAE &optical & 74.13&	83.75&	79.67&	89.88&	93.74&	55.04&	71.00    &	60.87&	85.18 \\
        SpectralGPT &optical & 89.07&	94.03&	93.17&	94.94&	97.44&	81.02&	89.52&	87.47&	91.66 \\
        S12-MoCo &optical & 89.26&	94.14&	93.26&	95.07&	97.47&	81.37&	89.73&	87.64&	91.92 \\
        S12-DINO  &optical& 88.61&	93.75&	92.78&	94.79&	97.31&	80.25&	89.04&	86.73&	91.48 \\
        S12-MAE  &optical & 87.79&	93.25&	91.69&	94.99&	97.14&	78.79&	88.13&	84.41&	92.2 \\
        S12-Data2Vec &optical & 88.15&	93.47&	92.48&	94.54&	97.19&	79.44&	88.54&	86.17&	91.05 \\
        \midrule
        UNet Baseline &  optical& \textbf{91.42} & \textbf{95.40}&	\underline{94.24}&	 \textbf{96.65} &  \textbf{98.03}&	 \textbf{85.05}&	 \textbf{91.92}&	\underline{89.18}&	 \textbf{94.84} \\
        ViT Baseline &optical & 87.66 &	93.17&	91.77&	94.71&	97.11 &	78.56&	87.99&	84.66&	91.60 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}
